A Simple Explanation for the Observed Power Law Distribution of Line Intensity in Complex Many-Electron Atoms

It has long been observed that the number of weak lines from many-electron atoms follows a power law distribution of intensity. While computer simulations have reproduced this dependence, its origin has not yet been clarified. Here we report that the combination of two statistical models -- an exponential increase in the level density of many-electron atoms and local thermal equilibrium of the excited state population -- produces a surprisingly simple analytical explanation for this power law dependence. We find that the exponent of the power law is proportional to the electron temperature. This dependence may provide a useful diagnostic tool to extract the temperature of plasmas of complex atoms without the need to assign lines.

==> latexmkrc <==
#!/usr/bin/perl
$latex         = 'pdflatex %O -src-specials -shell-escape -interaction=nonstopmode -synctex=1 powerlaw_spectra';
$bibtex        = 'pbibtex %O %B';
$dvipdf        = 'dvipdfmx %O -o %D powerlaw_spectra';
$pdf_mode      = 3; # use dvipdfmx

# Use SumatraPDF and atom inverse search
# $pdf_previewer = '"C:\Program Files\SumatraPDF\SumatraPDF.exe" -reuse-instance -inverse-search "\"%USERPROFILE%\AppData\Local\atom\bin\atom.cmd\" \"%f:%l\"" %O %S';

# if you do not need to preview in -pvc option (preview document and countinuously update mode)
# $pdf_previewer = 'exit';

